On Large Language Model Continual Unlearning

While large language models have demonstrated impressive performance across various domains and tasks, their security issues have become increasingly severe. Machine unlearning has emerged as a representative approach for model safety and security by removing the influence of undesired data on the target model. However, these methods do not sufficiently consider that unlearning requests in real-world scenarios are continuously emerging, especially in the context of LLMs, which may lead to accumulated model utility loss that eventually becomes unacceptable. Moreover, existing LLM unlearning methods often ignore previous data access limitations due to privacy concerns and copyright protection. Without previous data, the utility preservation during unlearning is much harder. To overcome these challenges, we propose the OOO framework that includes an Orthogonal low-rank adapter (LoRA) for continually unlearning requested data and an Out-Of-Distribution (OOD) detector to measure the similarity between input and unlearning data. The orthogonal LoRA achieves parameter disentanglement among continual unlearning requests. The OOD detector is trained with a novel contrastive entropy loss and utilizes a glocal-aware scoring mechanism. During inference, our OOO framework can decide whether and to what extent to load the unlearning LoRA based on the OOD detector's predicted similarity between the input and the unlearned knowledge. Notably, OOO's effectiveness does not rely on any retained data. We conducted extensive experiments on OOO and state-of-the-art LLM unlearning methods across three tasks and seven datasets. The results indicate that OOO consistently achieves the best unlearning effectiveness and utility preservation, especially when facing continuous unlearning requests. The source codes can be found at https://github.com/GCYZSL/O3-LLM-UNLEARNING.

==> sections/a.tex <==
\section{Problem Formulation}
\kz{problem formulation needs to be rewritten. Make the continual unlearning setting clear, especially about the data}

For a target LLM $M$ parameterized on $\Theta$, we consider a sequence of continually arriving unlearning requests with corresponding datasets with $N^{\mathrm{U}, t}$ samples, i.e., $\{\mathcal{D}^{\mathrm{U}, t}\}_{t=1}^T$ where $\mathcal{D}^{\mathrm{U}, t} = \{\bm{x}_i \| \bm{x}_i \sim \mathcal{P}_\mathcal{X}^{\mathrm{U}, t}\}_{i=1}^{N^{\mathrm{U}, t}}$ and $\mathcal{P}_\mathcal{X}^{\mathrm{U}, t}$ is the input marginal distribution. Each unlearning request corresponds to a task with the training data characterized by the input $\mathcal{P}^t_\mathcal{X}$ and label distributions $\mathcal{P}^t_\mathcal{Y}$. Traditional unlearning approaches always assume a retained dataset drawn from a distribution $\mathcal{P}^{\mathrm{R}, t}_\mathcal{X}$ disjoint from the unlearning one $\mathcal{P}^{\mathrm{U}, t}_\mathcal{X}$, i.e., $\mathrm{supp}(\mathcal{P}^{\mathrm{R}, t}_\mathcal{X}) = \mathrm{supp}(\mathcal{P}^{t}_\mathcal{X}) \setminus \mathrm{supp}(\mathcal{P}^{\mathrm{U}, t}_\mathcal{X})$ where $\mathrm{supp}(\cdot)$ denotes the support set of a distribution, to retain the model performance on the original training distribution. In this case, the objective of continual unlearning for LLM is
\begin{equation}
\begin{aligned}
    \sum_{t=1}^T \min_{\Theta^t}\mathbf{I}(M_{\bm{x} \sim \mathcal{P}_{\mathcal{X}}^{\mathrm{U}, t}}(\bm{x}, \Theta) ; M^t_{\bm{x} \sim \mathcal{P}_{\mathcal{X}}^{\mathrm{U}, t}}(\bm{x}, \Theta^t)), \,\sum_{t=1}^T \max_{\Theta^t}\mathbf{I}(M_{\bm{x} \sim \mathcal{P}_{\mathcal{X}}^{\mathrm{R}, t}}(\bm{x}, \Theta) ; M^t_{\bm{x} \sim \mathcal{P}_\mathcal{X}^{\mathrm{R}, t}}(\bm{x}, \Theta^t)),
\end{aligned}
\end{equation}
where $M^t$ parameterized on $\Theta^t$ represents the target model during and after unlearning on the $t$-th unlearning set $\mathcal{D}^{\mathrm{U}, t}$, and $\mathbf{I}(\cdot;\cdot)$ calculates the mutual information between two random variables.  

% $\mathcal{P}_\mathcal{X}^{\mathrm{R}, t}$ here is the input marginal distribution of the retained training dataset though it is unavailable during unlearning, and it is disjoint with previous unlearning requests and includes the marginal distribution of future unlearning requests, i.e., $\forall i \in [1, t], \mathrm{supp}(\mathcal{P}_\mathcal{X}^{\mathrm{U}, i}) \cap \mathrm{supp}(\mathcal{P}_\mathcal{X}^{\mathrm{R}, t}) = \emptyset$ and $\forall i \in (t, T], \mathrm{supp}(\mathcal{P}_\mathcal{X}^{\mathrm{U}, i}) \subset \mathrm{supp}(\mathcal{P}_\mathcal{X}^{\mathrm{R}, t})$.

% \subsection{System Goals}
% \subsubsection{Unlearning Scenarios} 
% This work considers three application scenarios of unlearning for LLMs. 
% \begin{itemize}[leftmargin=*]
%     \item There are some malicious, toxic, and harmful samples in the training data of the target model. Such data can incur model performance degradation, implant harmful backdoors, and disclose model and data privacy. This scenario happens when encountering errors during data collection and labeling as well as adversarial attacks during model training and tuning. In this case, unlearning can be leveraged to remove these malicious samples to mitigate their impact on the model and legal data.
%     \item LLMs may provide various services including question-answering, personal dialog, artistic creation, etc. The performance of LLMs on these tasks relies on a large volume of data that is often highly related to individual privacy and intellectual property. Although people may not initially know how their data was included in the LLM training, once they become aware, they may request the data to be deleted from the LLM through unlearning. For example, writers can request data deletion if they find ChatGPT has learned their literature without authorization, and daily users can request the removal of their dialog history with ChatGPT.
%     \item As time goes on, the knowledge that has been learned by an LLM may become incorrect, outdated, or biased, which hurts the model performance. This is unavoidable as new knowledge and information evolve. In this case, unlearning can be used to correct and update such information to make sure that the LLM evolves accordingly as well.
% \end{itemize}


% biology 1192
% physics 595
% chemistry 403
% economics 237


% \subsubsection{Practicality}
% \label{sec_practicality}
% This work addresses the practicality of LLM unlearning in the following aspects.
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Data Availability.} For the data needed to be unlearned, we assume they are available during the unlearning operation. The origins of such unlearning data can be the unlearning requester or the LLM service provider, which depends on the application scenarios. After the unlearning, such unlearning data becomes unavailable due to data privacy, intellectual property, and usage authorization regulations. Similarly, the retained training dataset of the target LLM cannot be assumed to be entirely available during unlearning due to these regulations. In addition to the raw data, we assume there is no task label for the unlearning and retained datasets, though there might be some in practice. 
%     \item \textbf{Continual Unlearning.} In real-world applications, the LLM unlearning requests emerge continuously over time. For instance, attackers launch adversarial attacks when LLM continuously learns new data; daily users periodically want to delete dialog history; the knowledge becomes outdated and incorrect over time. To deal with these continuous unlearning requests, the LLM unlearning should be operated effectively and, more importantly, alleviate the cumulative catastrophic utility loss. The utility implies that the LLM's performance on other tasks that are disjoint from the unlearning requests.
%     \item \textbf{Computation Efficiency.} Although existing LLM unlearning methods may adopt various approximation approaches rather than retraining to reduce the computation overhead, there are further efforts that can enhance efficiency. Given that LLMs are typically built upon large-scale transformers, unlearning does not have to be conducted across the entire model. Instead, a better choice is to adopt some parameter-efficient fine-tuning (PEFT) strategies~\cite{peft_1, hu2021lora} to reduce the computation cost. Moreover, reducing or eliminating the use of the retained dataset also improves efficiency, especially considering the challenges in accessing the entire retained training data due to various regulations mentioned above. Adopting the PEFT strategy at the model level and minimizing the use of the retained dataset at the data level is particularly beneficial for efficiency, given the cumulative computation overhead in responding to continual unlearning requests.
% \end{itemize}





% \subsection{Motivation}
% \cy{Add motivation}

==> sections/background.tex <==
\section{Background}

\subsection{Machine Unlearning}
Standard machine unlearning~\cite{machine_unlearning} ensures the ``right to be forgotten"~\cite{gdpr2018general, ccpa} and allows individuals to request the deletion of their data from the machine learning service provider. Formally speaking, we assume the data that needs to be unlearned is termed as $\mathcal{D}^\mathrm{U} \!=\! \{(\bm{x}_i, y_i) \| \bm{x}_i \!\sim\! \mathcal{P}_\mathcal{X}^\mathrm{U}, y_i \!\sim\! \mathcal{P}_\mathcal{Y}^\mathrm{U}\}_{i=1}^{N^\mathrm{U}}$ ($N^\mathrm{U}$ is the sample quantity). $\mathcal{P}_\mathcal{X}^\mathrm{U}$ and $\mathcal{P}_\mathcal{Y}^\mathrm{U}$ are the input and label marginal distributions of the unlearning set, respectively. Note that $\mathcal{D}^\mathrm{U}$ naturally comes from the original training dataset of the target model $M_\Theta$ that is parameterized on $\Theta$. Moreover, we denote the retained training dataset without $\mathcal{D}^\mathrm{U}$ as $\mathcal{D}^\mathrm{R} = \{(\bm{x}_i, y_i) \| \bm{x}_i \!\sim\! \mathcal{P}_\mathcal{X}^\mathrm{R}, y_i \!\sim\! \mathcal{P}_\mathcal{Y}^\mathrm{R}\}_{i=1}^{N^\mathrm{R}}$. To achieve effective unlearning, the most direct way is to retrain another randomly initialized model from scratch with the retained dataset $\mathcal{D}^\mathrm{R}$. However, when the target model becomes larger and requires more training data, such training from scratch consumes a large volume of computation resources. Many approximation approaches have been proposed to reduce such high computational overhead, which we will discuss in Section~\ref{sec_related_works}. These approaches share the same objective, which is to remove the memorization about $\mathcal{D}^\mathrm{U}$ from the target model $M_\Theta$ while retaining the performance on $\mathcal{D}^\mathrm{R}$,
\begin{equation}
\begin{aligned}
    &\min_{\Theta^\prime}\mathbf{I}(M_{\bm{x}\in\mathcal{D}^\mathrm{U}}(\bm{x}, \Theta) ; M^\prime_{\bm{x}\in\mathcal{D}^\mathrm{U}}(\bm{x}, \Theta^\prime)) \\
    &\max_{\Theta^\prime}\mathbf{I}(M_{\bm{x}\in\mathcal{D}^\mathrm{R}}(\bm{x}, \Theta) ; M^\prime_{\bm{x}\in\mathcal{D}^\mathrm{R}}(\bm{x}, \Theta^\prime)),
\end{aligned}
\end{equation}
where $\mathbf{I}(\cdot;\cdot)$ calculates the mutual information between two random variables and $M^\prime$ parameterized on $\Theta^\prime$ denotes the target model during and after unlearning.

\subsection{Large Language Models}
Large Language Models (LLMs) have revolutionized the field of natural language processing (NLP) by achieving unprecedented performance on a wide range of tasks~\cite{wang2024survey, llm_survey_1}. Among the mainstream LLMs, models such as Google's Gemini~\cite{team2023gemini} and Meta's LLaMA-3~\cite{llama3modelcard} have set new benchmarks in various applications. These models are built with well-crafted architectures and have been trained on vast amounts of data, enabling them to understand and generate human-like text with remarkable quality.

The training data for LLMs is vast and diverse. For instance, GPT-3 was trained on 45 TB of text data~\cite{gpt3}, which includes content from Wikipedia, Common Crawl, and various repositories. Such massive data allows the models to capture the intricacies of human language, covering a wide range of topics. The scale of training data ensures that LLMs are exposed to diverse linguistic patterns and contextual nuances, which are critical for their performance on various tasks, including translation, sentiment analysis, and question-answering. Their ability to generate coherent and contextually relevant text makes them valuable tools for applications like content creation, customer support, and educational tools.

The underlying architecture of LLMs is predominantly based on the transformer model. Introduced by Vaswani et al.~\cite{vaswani2017attention}, the transformer architecture is characterized by using self-attention mechanisms and parallel processing capabilities. The basic components of the transformer model include an encoder and a decoder, each comprising multiple layers of attention and feed-forward neural networks. The self-attention mechanism enables the model to weigh the importance of different words in a sentence relative to each other, capturing long-range dependencies and contextual relationships effectively. In recent years, the decoder-only architecture (GPT~\cite{gpt3}, LLaMA~\cite{llama3modelcard, touvron2023llama2}) has become more popular than the encoder-decoder (T5~\cite{t5}, BART~\cite{lewis2020bart}) or encoder-only (BERT~\cite{devlin2019bert}) design, thus being adopted by the mainstream LLMs.



==> sections/discussion.tex <==
\section{Discussion}
\subsection{Future Work for Unlearning Knowledge Detection}
A direct improvement related to unlearning knowledge detection lies in the inference stage. In the inference phase of \OOO{} framework, we need to feed the testing data into each OOD detector to calculate the likelihood of belonging to previous unlearning distributions. In practical system deployment, we can parallelize this process to enhance efficiency~\cite{parallel_inference}.

In our implementation, the OOD detector backbone uses the encoder-only Roberta model. Although this model can extract high-quality representations, its performance is still limited when faced with complex inputs compared to larger-scale language models. Therefore, we consider directly using the target LLM to detect unlearning knowledge. This approach is feasible because, in the \OOO{} framework, we use LoRA as an external module to achieve unlearning, and the original target LLM is available for inference. We should gain the following benefits if we replace the OOD detector backbone with an LLM. First, LLMs can better capture subtle text differences, improving OOD detection performance. Second, smaller language models like Roberta cannot effectively extract contextual information from complex and long contexts. Thus, if an unlearning request correlates the contextual information, such as the individual users' request to unlearn specific topics from their chat history with ChatGPT, Roberta-based OOD detection cannot achieve this. In contrast, LLMs can extract contextual information well~\cite{long_context}, supporting more fine-grained OOD detection and more accurate ID data localization. Finally, using LLMs for OOD detection might eliminate the need for fine-tuning with ID data, as Uppaal et al.~\cite{no_need_fine_tune} suggested that LLMs could provide accurate OOD detection predictions for text classification without any fine-tuning. This could further improve our framework's efficiency. However, using LLMs for OOD detection might require dedicated improvements to the scoring mechanism because mainstream LLMs now use a decoder-only architecture, which works by predicting the next token. In this case, the representation output by each attention layer of the LLM is likely to be highly inconsistent in terms of token quantity and distribution. Therefore, whether our design based on layer-wise token average representation (Section~\ref{sec_scoring_mechanism}) is suitable for LLMs requires further research.

\subsection{Data Selection for LLM Utility Preservation}
\label{sec_data_selection_utility}
In the real world, we often edit LLMs for various purposes, such as knowledge unlearning. However, this model editing leads to uncertain and unpredictable changes in the capabilities of the LLM~\cite{qifine, sequential_hurt, sequential_hurt_2}. For instance, recent studies have shown that model editing for a single specific task can cause performance degradation in seemingly unrelated tasks. This phenomenon is more pronounced in sequential or continual model editing~\cite{sequential_hurt, sequential_hurt_2}. To address this issue, similar to leveraging a retained dataset to preserve model utility in LLM unlearning~\cite{unlearning_motivation_1}, the intuitive approach is to identify which tasks and data distributions are most affected and then replay some representative data on the LLM~\cite{replay}. However, identifying these tasks and data distributions on an LLM is extremely challenging~\cite{localization_challenging, localize_dif_1, localize_dif_2}. For example, to select suitable retained data for utility preservation in LLM unlearning, we might utilize some interpretable machine learning (ML) techniques~\cite{interpretable_ML} to locate the neurons activated by the unlearning data. Based on these identified activated neurons, we could retrieve similar data to be used as the retained data. However, current interpretable ML techniques typically only achieve neuron localization for specific model attributes, such as adversarial robustness~\cite{localize_adversarial} or differential privacy~\cite{localize_dp}. For the fine-grained tasks and data distributions corresponding to unlearning requests, neuron localization is either inaccurate or inconsistent in granularity. Therefore, effective data selection to preserve LLM utility during unlearning is research-worthy.


